Adaptive Control of Distributed Energy Resources for Distribution Grid Voltage Stability

Volt-VAR and Volt-Watt functionality in photovoltaic (PV) smart inverters provide mechanisms to ensure system voltage magnitudes and power factors remain within acceptable limits. However, these control functions can become unstable, introducing oscillations in system voltages when not appropriately configured or maliciously altered during a cyberattack. In the event that Volt-VAR and Volt-Watt control functions in a portion of PV smart inverters in a distribution grid are unstable, the proposed adaptation scheme utilizes the remaining and stably-behaving PV smart inverters and other Distributed Energy Resources to mitigate the effect of the instability. The adaptation mechanism is entirely decentralized, model-free, communication-free, and requires virtually no external configuration. We provide a derivation of the adaptive control approach and validate the algorithm in experiments on the IEEE 37 and 8500 node test feeders.

==> intro_original.tex <==
\section{Introduction}
\label{sec:introduction}

Increasing adoption of Distributed Energy Resources (DER), specifically rooftop photovoltaic (PV) generation systems, is challenging many conventionally-held models and practices regarding the electric power system's operation.  While the presence of DER gives individuals and communities the ability to self-generate at least a portion of their load, they also make proper management of the power system more difficult as many DER are not utility-owned/operated.

Emerging standards \cite{IEEE_1547, rule21, inverter2016} are encouraging the use of device-level modulation of active and reactive power injection in response to local grid conditions.  These autonomous control functions allow DER to quickly correct undesirable voltages and power factors at the point of injection and (in theory) alleviate the need for a response from the grid managing entity.

Although these autonomous control functions, specifically smart inverter Volt-VAR (VV) and Volt-Watt (VW) controllers, are well-intentioned, numerous works have emerged showing that proper configuration of individual devices is crucial for the stable operation of the DER population.  Authors in \cite{jahangiri2013distributed} discussed the phenomenon of \textquote{hunting} in voltages in systems with VV control. Authors in \cite{farivar2013equilibrium} modeled the interaction between system voltage magnitudes and PV inverter VV functions as a feedback control loop, thus explicitly tied the slopes of VV controllers of inverters to unstable (highly oscillatory) reactive power injections.  Although the instability threshold depends on the network's specifics, instability is reached when the slopes of the VV control curves become too steep. Numerous other works also modeled the inverter/grid interaction as a first-order feedback controller and arrived at similar stability conditions \cite{zhou2016local, braslavsky2017voltage, bakerNetwork2017, eggli2020stability, saha2020lyapunov}. Moreover, adaptive control approaches have been previously been applied to improve the interaction of PV systems and the electric grid.

While it is possible that instabilities may arise naturally in a system (due to system reconfiguration, poor parameterizations of VV/VW functions, or intermittency in PV penetration), the remote update capability of many smart inverter devices presents a vulnerability that a malicious entity could purposefully exploit to destabilize the smart inverter/grid interaction \cite{sahoo2019cyber}. Security researchers have identified exploitable vulnerabilities in deployed inverter firmware \cite{practical2017}, foreign nations are actively targeting the US bulk power system \cite{russian2018}, and in at least one instance, a US inverter control system has been successfully attacked \cite{risks2019}.  An excellent example of the extent to which aggregations of smart inverters can be remotely updated was illustrated in Hawaii, where local utilities worked with a smart inverter vendor to remotely update the autonomous control functions of 800,000 inverters in a single day \cite{spectrum2015}.  

In this work, we propose an adaptive control approach to adjust the VV/VW control functions of stable PV systems (which we will henceforth refer to as \emph{non-compromised}) and active/reactive power injections of other DER (e.g., battery storage systems) to mitigate voltage instabilities in the system.  A high-level diagram of the adaptive control approach's role is shown in Fig. \ref{fig:devices_block_diagram}, which depicts three classes of devices in feedback with the electric grid.  All devices inject active $p$ and reactive $q$ power into the grid and measure the grid voltage $v$ at their point of interconnection.  While a portion of smart inverters in the system with VV/VW are unstable, a subset of smart inverters and other DER capable of directly injecting power into the grid can be adjusted by the proposed adaptive control via the signal $u$.  When applied to control a direct power injection device, $u$ is the additional amount of active/reactive power injected (or consumed, if $u$ changes sign) into the grid.  When controlling PV smart inverter VV or VW controllers (or both), $u$ is a voltage bias that is added to the measured grid voltage magnitude.  Note that we explicitly assume that unstable PV smart inverter systems are not controllable as they may have been, in the worst case, compromised via a cyberattack and should be considered unreliable for control.  

\begin{figure}[h]
\includegraphics[width=0.4\textwidth]{figures/multiple_devices.png}
\caption{Block diagram of controllable devices.}
\label{fig:devices_block_diagram}
\end{figure}

The controller derived herein belongs to a class of algorithms known as Model Reference Adaptive Controllers (MRAC) \cite{astrom2008adaptive} that utilize a stable \emph{reference model} to compare to the unstable plant.  The adaptation mechanism is designed via Lyapunov analysis to drive the error between the plant and the reference to 0 asymptotically.  
  Ghasemi et al. \cite{GHASEMI2016prevention} consider control law to adapt PV reactive power injection for loss minimization and overvoltage prevention.  In a closely related work, Singhal et. al. \cite{singhal2019real} translate the smart inverter Volt-VAr curves for steady state error reduction and flatten Volt-VAr curves to mitigate instabilities.  While stretching/flattening VV curves proved effective in reducing oscillations in situations considered in the paper, the strategy has two drawbacks: 1) it does not account for the scenario where a subset of the PV devices in a given system are solely responsible for creating instabilities and are not controllable, and 2) the algorithm requires the use of ``correction factors" which are estimated offline based on sensitivity analysis and engineering judgement.  These correction factors would need to be estimated by an entity with complete grid knowledge and relayed to individual smart inverters, requiring a substantial communications overhead.  Such a system also constitutes a cybersecurity vulnerability as discussed earlier.  Additionally, correction factor computation would need to be carried out periodically as new PV systems are installed or the grid is reconfigured.

The main contribution of this paper is the construction of an adaptive control scheme for adjusting both PV smart inverter Volt-VAR and Volt-Watt settings, and power injections of a wide variety of other classes of DER, \emph{in real time}.  The approach is further distinguished in that it employs the low pass filtered AC grid voltage magnitude measured by the PV system/DER as the as a proxy for the stable reference model.  This particular choice of reference model makes the algorithm decentralized, (system) model-free, and communications-free.  The adaptation law complies with existing smart inverter standards \cite{IEEE_1547,rule21, inverter2016}, allowing for a decentralized implementation directly within the smart inverter or DER with minimum additional investment.  The control law generalizes to both controllable PV smart inverter systems and devices capable of direct power injection (the adaptation law is identical for both device classes).  Asymptotic stability of the control law is proven with rigor and demonstrated in time series simulations of unbalanced distribution systems.  

This paper is organized as follows.  In Section \ref{sec:preliminaries} we briefly derive a linear balanced power flow model for subsequent control design and discuss smart inverter dynamic modeling assumptions.  In Section \ref{sec:stability}, we analyze the stability of the smart inverter VV/VW control functions in feedback with the electric grid.  Derivation of the adaptive control scheme is presented in Section \ref{sec:control_design}.  Simulation results showing the effectiveness of the controller in \emph{unbalanced} systems are discussed in Section \ref{sec:results}.  Finally, concluding remarks are presented in Section \ref{sec:conclusions}.

==> stability_analysis.tex <==
\section{Stability Analysis}
\label{sec:stability}

In this section we explore the stability of smart inverters, modeled by Fig. \ref{fig:inverter_block_diagram}, connected to the distribution grid.  Without loss of generality, we assume the presence of a VV and VW capable smart inverter at each node in the system.  Under the additional assumption that active and reactive power consumption due to system loads change slowly with respect to inverter control actions, \eqref{eq:lindistflow2} can be recast in the following form:
\begin{align}
    \mathbf{v} = \mathbf{Z}\mathbf{s} + \underbrace{\mathbf{v_{0}} - \mathbf{Z}\mathbf{s^{c}}}_{\mathbf{\bar{v}}} \label{eq:lindistflow3},
\end{align}
% \begin{gather}
%     \mathbf{v} = \mathbf{R}\mathbf{p} + \mathbf{X}\mathbf{q} +  \underbrace{\mathbf{v_{0}} - \mathbf{R}\mathbf{p^{c}} - \mathbf{X}\mathbf{q^{c}}}_{\mathbf{\bar{v}}} \label{eq:lindistflow2},
% \end{gather}
\noindent where the superscript has been dropped from $\mathbf{s}$ for convenience and $\mathbf{\bar{v}}$ is treated as constant. Consistent with Fig. \ref{fig:inverter_block_diagram}, the dynamics of the inverter consist of nonlinear Volt-VAR \& Volt-Watt controllers in series with first order low pass filters can be expressed as \cite{saha2020lyapunov}:
\begin{subequations}
\begin{align}
    \mathbf{T}\mathbf{\dot{s}} &= \mathbf{f}(\mathbf{v}) -\mathbf{s}, \label{eq:sdot}\\
    \mathbf{v} &= \mathbf{Z}\mathbf{s} + \mathbf{\bar{v}} \label{eq:v}
\end{align}
\end{subequations}
\noindent where $\mathbf{T} \in \mathbb{R}^{2n \times 2n}$ is a diagonal and positive definite matrix that collects low pass filter time constants.  

In this model, $\mathbf{f}(\mathbf{v}) = [\mathbf{f}_{p}(\mathbf{v}), \mathbf{f}_{q}(\mathbf{v})]^{T}$ is the collection of inverter VV and VW functions at each node in $\mathcal{G}$, where:
\begin{subequations}
\begin{align}
    \mathbf{f}_{p}( \mathbf{v}) &= [f_{p,1}(v_{1}), \ldots, f_{p,n}(v_{n})]^{T} \label{eq:fpi}\\
    \mathbf{f}_{q}( \mathbf{v}) &= [f_{q,1}(v_{1}), \ldots, f_{q,n}(v_{n})]^{T} \label{eq:fqi},
\end{align}
\end{subequations}

\noindent where, according to Assumptions \ref{assumption:f_1}-\ref{assumption:f_2}, both $f_{p,i}(v_{i})$ and $f_{q,i}(v_{i})$ are locally Lipschitz with constants $C_{p,i}$ and $C_{q,i}$, respectively.  Define the matrices
\begin{subequations}
    \begin{align}
        \mathbf{C}_{p} &= \text{diag}([C_{p,1}, \ldots, C_{p,n}])\\
        \mathbf{C}_{q} &= \text{diag}([C_{q,1}, \ldots, C_{q,n}])\\
        \mathbf{C}_{s} &= \mqty[ \mathbf{C}_{p} & \mathbf{C}_{q}]^{T}.
    \end{align}
\end{subequations}
    
The following proposition ties the stability of \eqref{eq:sdot} - \eqref{eq:v} to the system impedances, $\mathbf{Z}$, and $\mathbf{C}_{s}$.

\begin{proposition}
\label{prop:direct}
Let $\mathbf{M} \in \mathcal{R}^{2n \times 2n}$ be a positive definite and symmetric matrix.  The system of \eqref{eq:sdot} - \eqref{eq:v} is asymptotically stable if:
\begin{equation}
    -\underline{\lambda} + \overline{\lambda}  \norm{ \mathbf{C}_{s}\mathbf{Z}}_{2} \le 0 \label{eq:stab_cond},
\end{equation}

\noindent where $\underline{\lambda} = \lambda_{\min}(\mathbf{MT}^{-1})$ and $\overline{\lambda} = \lambda_{\max}(\mathbf{MT}^{-1})$.
\end{proposition}

\begin{proof}
    Noting the equilibrium $\mathbf{s}^{*}$ of \eqref{eq:sdot} is 
    \begin{equation}
            \mathbf{0} = \mathbf{f}(\mathbf{Z}\mathbf{s}^{*} + \mathbf{\bar{v}}) -\mathbf{s}^{*}\label{eq:eqpoint},
    \end{equation}
    
    \noindent define the shifted set of coordinates $\Delta \mathbf{s} = \mathbf{s} - \mathbf{s}^{*}$ which translate the equilibrium to the origin.  The dynamics in the new coordinate system are:
    \begin{equation}
        \mathbf{T}\Delta\mathbf{\dot{s}} = \mathbf{f}(\mathbf{Z}\Delta\mathbf{s} + \mathbf{Z}\mathbf{s}^{*} + \mathbf{\bar{v}}) - \mathbf{f}(\mathbf{Z}\mathbf{s}^{*} + \mathbf{\bar{v}}) -\Delta\mathbf{s} \label{eq:delsdot}.
    \end{equation}

Let $\mathbf{\alpha} = \mathbf{Z}\mathbf{s}^{*} + \mathbf{\bar{v}}$.  Using the Lyapunov function $V = \frac{1}{2}\Delta \mathbf{s}^{T}\mathbf{M}\Delta \mathbf{s}$, the derivative of the state trajectories of \eqref{eq:delsdot} along $V$ are:
\begin{subequations}
    \begin{align}
        \dot{V} &= \Delta \mathbf{s}^{T} \mathbf{MT}^{-1}\Big( \mathbf{f}(\mathbf{Z} \Delta \mathbf{s} + \mathbf{\alpha}) - \mathbf{f}(\mathbf{\alpha}) \Big) \nonumber \\
        & - \frac{1}{2}\Delta \mathbf{s}^{T} \big( \mathbf{T}^{-1}\mathbf{M} + \mathbf{MT}^{-1}\big)\Delta \mathbf{s} \label{eq:ve_dot1}\\
        &\le \begin{Vmatrix}
            \Delta \mathbf{s}
        \end{Vmatrix}_{2} \cdot \begin{Vmatrix}
            \mathbf{MT}^{-1}
            \end{Vmatrix}_{2} \cdot \begin{Vmatrix}
            \mathbf{f}(\mathbf{Ze}_{s} + \mathbf{\alpha}) - \mathbf{f}(\mathbf{\alpha})
        \end{Vmatrix}_{2} \nonumber \\
        & -\begin{Vmatrix}
            \mathbf{MT}^{-1}
            \end{Vmatrix}_{2} \cdot \begin{Vmatrix}
            \Delta \mathbf{s}
        \end{Vmatrix}_{2}^{2}\label{eq:ve_dot2}\\
        &\le \begin{Vmatrix}
            \Delta \mathbf{s}
        \end{Vmatrix}_{2} \cdot \begin{Vmatrix}
            \mathbf{MT}^{-1}
            \end{Vmatrix}_{2} \cdot \begin{Vmatrix}
            \mathbf{C}_{s}\mathbf{Z}\Delta \mathbf{s}
        \end{Vmatrix}_{2} \nonumber \\
        &  -\begin{Vmatrix}
            \mathbf{MT}^{-1}
            \end{Vmatrix}_{2} \cdot \begin{Vmatrix}
            \Delta \mathbf{s}
        \end{Vmatrix}_{2}^{2} \label{eq:ve_dot3}\\
        &\le \qty(-\underline{\lambda} + \overline{\lambda}\begin{Vmatrix}
            \mathbf{C}_{s}\mathbf{Z}
        \end{Vmatrix}_{2})\begin{Vmatrix}
            \Delta \mathbf{s}
        \end{Vmatrix}_{2}^{2} \label{eq:ve_dot4},
    \end{align}
\end{subequations}

\noindent where \eqref{eq:ve_dot3} follows from the fact that $\mathbf{f}$ is a Lipschitz nonlinearity with Lipschitz constant $\mathbf{C}_{s}$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this section we explore the stability of smart inverters, modeled by Fig. \ref{fig:inverter_block_diagram}, connected to the distribution grid.  Without loss of generality, we assume the presence of a VV and VW capable smart inverter at each node in the system.  Under the additional assumption that active and reactive power consumption change slowly with respect to inverter control actions, \eqref{eq:lindistflow2} can be recast in the following form:
% \begin{align}
%     \mathbf{v} = \mathbf{Z}\mathbf{s} + \underbrace{\mathbf{v_{0}} - \mathbf{Z}\mathbf{s^{c}}}_{\mathbf{\bar{v}}} \label{eq:lindistflow3},
% \end{align}

% % \begin{gather}
% %     \mathbf{v} = \mathbf{R}\mathbf{p} + \mathbf{X}\mathbf{q} +  \underbrace{\mathbf{v_{0}} - \mathbf{R}\mathbf{p^{c}} - \mathbf{X}\mathbf{q^{c}}}_{\mathbf{\bar{v}}} \label{eq:lindistflow2},
% % \end{gather}

% \noindent where the superscript has been dropped from $\mathbf{s}$ for convenience and $\mathbf{\bar{v}}$ is treated as constant. Consistent with Fig. \ref{fig:inverter_block_diagram}, the following formulation explicitly models the dynamics associated with measuring the instantaneous voltage (Eq. \eqref{eq:lindistflow3}) \emph{and} computing new active/reactive power injections.  Both processes are modeled using first order low pass filters.  Letting the vector $\mathbf{v}$ denote the collection of \emph{measured} voltages, the inverter dynamics can be expressed as:
% %Denote the vector of measured voltages as $\mathbf{v}_{m} \in \mathbb{R}^{n \times 1}$.  
% %Extending the structure of the DER Volt-VAR and Volt-Watt control schemes discussed in \cite{bakerNetwork2017}, \cite{farivar2013equilibrium}, \cite{braslavsky2017voltage}, \cite{SCHIFFER20142457},\cite{eggli2020stability} we model the dynamics of the measured voltage in feedback with the smart inverter control functions as a first order low pass filter:
% \begin{subequations}
% \begin{align}
%     \mathbf{T}_{v}\mathbf{\dot{v}} &= \mathbf{Z}\mathbf{s} + \mathbf{\bar{v}} - \mathbf{v} \label{eq:vdot},\\
%     \mathbf{T}_{s}\mathbf{\dot{s}} &= \mathbf{f}(\mathbf{v}) -\mathbf{s}, \label{eq:sdot}
% \end{align}
% \end{subequations}

% \noindent where $\mathbf{T}_{v} \in \mathbb{R}^{n \times n}$ and $\mathbf{T}_{s} \in \mathbb{R}^{2n \times 2n}$ are time constants of measurement and power injection update dynamics (diagonal and positive definite).  

% In this model, $\mathbf{f}(\mathbf{v}) = [\mathbf{f}_{p}(\mathbf{v}), \mathbf{f}_{q}(\mathbf{v})]^{T}$ is the collection of inverter VV and VW functions at each node in $\mathcal{G}$, where:
% \begin{subequations}
% \begin{align}
%     \mathbf{f}_{p}( \mathbf{v}) &= [f_{p,1}(v_{1}), \ldots, f_{p,n}(v_{n})]^{T} \label{eq:fpi}\\
%     \mathbf{f}_{q}( \mathbf{v}) &= [f_{q,1}(v_{1}), \ldots, f_{q,n}(v_{n})]^{T} \label{eq:fqi},
% \end{align}
% \end{subequations}

% \noindent where, according to Assumptions \ref{assumption:f_1}-\ref{assumption:f_2}, both $f_{p,i}(v_{i})$ and $f_{q,i}(v_{i})$ are locally Lipschitz with constants $C_{p,i}$ and $C_{q,i}$, respectively.  Define the matrices
% \begin{subequations}
%     \begin{align}
%         \mathbf{C}_{p} &= \text{diag}([C_{p,1}, \ldots, C_{p,n}])\\
%         \mathbf{C}_{q} &= \text{diag}([C_{q,1}, \ldots, C_{q,n}])\\
%         \mathbf{C}_{s} &= \mqty[ \mathbf{C}_{p} & \mathbf{C}_{q}]^{T}.
%     \end{align}
% \end{subequations}
    
% The following proposition ties the stability of \eqref{eq:vdot} - \eqref{eq:sdot} to the system impedances, $\mathbf{Z}$, and $\mathbf{C}_{s}$.

% \begin{proposition}
% \label{prop:direct}
% The system of \eqref{eq:vdot} - \eqref{eq:sdot} is asymptotically stable if:
% \begin{equation}
%     \norm{\mathbf{Z}\mathbf{C}_{s}}_{2} \le 1 \label{eq:stab_cond}
% \end{equation}
% \end{proposition}

% \begin{proof}
%     Noting the equilibrium $(\mathbf{v}^{*},\mathbf{s}^{*})$ of \eqref{eq:vdot} - \eqref{eq:sdot} is 
%     \begin{subequations}
%         \begin{align}
%             \mathbf{0} &= \mathbf{Z}\mathbf{s}^{*} + \mathbf{\bar{v}} - \mathbf{v}^{*}\label{eq:eqpoint1}\\
%             \mathbf{0} &= \mathbf{f}(\mathbf{v}^{*}) -\mathbf{s}^{*}\label{eq:eqpoint2},
%         \end{align}
%     \end{subequations}
    
%     \noindent define the shifted set of coordinates $\Delta\mathbf{v} = \mathbf{v} - \mathbf{v}^{*}$, $\Delta \mathbf{s} = \mathbf{s} - \mathbf{s}^{*}$ which translate the equilibrium to the origin.  The dynamics in the new coordinate system are:
%     \begin{subequations}
%     \begin{align}
%         \mathbf{T}_{v}\Delta\mathbf{\dot{v}} &= \Big(\mathbf{Z}\Delta\mathbf{s} -\Delta\mathbf{v}\Big) \label{eq:delvdot},\\
%         \mathbf{T}_{s}\Delta\mathbf{\dot{s}} &= \Big(\mathbf{f}(\Delta\mathbf{v} + \mathbf{v}^{*}) - \mathbf{f}(\mathbf{v}^{*}) -\Delta\mathbf{s}\Big) \label{eq:delsdot}.
%     \end{align}
% \end{subequations}

% Define the vector
% \begin{equation}
%     \mathbf{g}(\Delta\mathbf{v},\Delta\mathbf{s}) = \mqty[\mathbf{Z}\Delta\mathbf{s}\\ \mathbf{f}(\Delta\mathbf{v} + \mathbf{v}^{*}) - \mathbf{f}(\mathbf{v}^{*})].
% \end{equation}

% The 2-norm of the vector $\mathbf{g}$ can be expressed as:
% \begin{subequations}
%     \begin{align}
%         \norm{\mathbf{g}}_{2} &\le \begin{Vmatrix}
%             \mathbf{Z}\Delta\mathbf{s}
%         \end{Vmatrix}_{2} + 
%         \begin{Vmatrix}
%             \mathbf{f}(\Delta\mathbf{v} + \mathbf{v}^{*}) - \mathbf{f}(\mathbf{v}^{*})
%             \end{Vmatrix}_{2}\label{eq:g_1} \\
%         &\le \begin{Vmatrix}
%             \mathbf{Z}\Delta\mathbf{s}
%         \end{Vmatrix}_{2} + 
%         \begin{Vmatrix}
%             \mathbf{C}_{s} \Delta\mathbf{v}
%         \end{Vmatrix}_{2}\label{eq:g_2}\\
%         &= \begin{Vmatrix}
%             \begin{bmatrix}
%                     \mathbf{0}_{n\times n} & \mathbf{Z} \\
%                     \mathbf{C}_{s} & \mathbf{0}_{2n\times 2n} 
%             \end{bmatrix}\begin{bmatrix}
%                             \Delta\mathbf{v} \\
%                             \Delta \mathbf{s}
%                     \end{bmatrix}
%         \end{Vmatrix}_{2} \label{eq:g_3}\\
%         &\le \begin{Vmatrix}
%             \begin{bmatrix}
%                     \mathbf{0}_{n\times n} & \mathbf{Z} \\
%                     \mathbf{C}_{s} & \mathbf{0}_{2n\times 2n} 
%             \end{bmatrix}
%         \end{Vmatrix}_{2} \begin{Vmatrix}
%             \begin{bmatrix}
%                             \Delta\mathbf{v} \\
%                             \Delta \mathbf{s}
%                     \end{bmatrix}
%         \end{Vmatrix}_{2} \label{eq:g_4}.
%     \end{align}
% \end{subequations}

% Let $\Delta \mathbf{y} = [\Delta\mathbf{v}, \Delta \mathbf{s}]^{T}$.  The dynamics of \eqref{eq:delvdot} - \eqref{eq:delsdot} can be expressed in terms of $\Delta \mathbf{y}$:
% \begin{equation}
%     \mathbf{T}\Delta \mathbf{\dot{y}} = \Big( -\Delta \mathbf{y} + \mathbf{g}(\Delta \mathbf{y})\Big) \label{eq:delydot},
% \end{equation}

% \noindent where $\mathbf{T} = \text{diag}([\mathbf{T}_{v}, \mathbf{T}_{s}])$.  

% Using the Lyapunov function $V = \frac{1}{2}\Delta \mathbf{y}^{T}\mathbf{T}\Delta \mathbf{y}$, the derivative of the state trajectories of \eqref{eq:delydot} along $V$ are:
% \begin{subequations}
%     \begin{align}
%         \dot{V} &= -\Delta \mathbf{y}^{T} \Delta \mathbf{y} + \Delta \mathbf{y}^{T}\mathbf{g}(\Delta \mathbf{y}) \label{eq:vdot1}\\\
%         &\le \norm{\Delta \mathbf{y}}^2_2 + \norm{\Delta \mathbf{y}}_2 \norm{\mathbf{g}(\Delta \mathbf{y})}_2 \label{eq:vdot2} \\
%         % &\le -\begin{Vmatrix}
%         %     \Delta \mathbf{y}
%         % \end{Vmatrix}_{2}^{2} + \begin{Vmatrix}
%         %     \Delta \mathbf{y}
%         % \end{Vmatrix}_{2}\begin{Vmatrix}
%         %     \mathbf{g}(\Delta \mathbf{y})
%         % \end{Vmatrix}_{2} \label{eq:vdot2} \\
%         &\le \qty(-1- \norm{\mqty[\mathbf{0}_{n\times n} & \mathbf{Z} \\ \mathbf{C}_{s} & \mathbf{0}_{2n\times 2n}  ]}) \norm{\Delta \mathbf{y}}^2_2 \label{eq:vdot3}, 
%         % &\le \Bigg( -1 + \begin{Vmatrix}
%         %     \begin{bmatrix}
%         %             \mathbf{0}_{n\times n} & \mathbf{Z} \\
%         %             \mathbf{C}_{s} & \mathbf{0}_{2n\times 2n} 
%         %     \end{bmatrix}
%         % \end{Vmatrix}_{2}\Bigg)\begin{Vmatrix}
%         %     \Delta \mathbf{y}
%         % \end{Vmatrix}_{2}^{2} \label{eq:vdot3},
%     \end{align}
% \end{subequations}

% \noindent where the terms in parenthesis can be equivalently expressed as $\norm{\mathbf{Z}\mathbf{C}_{s}}_{2} \le 1$.
% \end{proof}
